Locating and Controlling Implicit Personalization in Large Language Models

Large language models (LLMs) often shift their outputs in response to implicit demographic cues even when users never state a demographic identity. Previous work has documented this behavior, but the connection between these behavioral changes and the model's internal activations remains unclear. Using matched cued and neutral conversations across five LLMs, we establish that a localized internal activation signal tracks changes in recommendations, with correlations up to r=0.87. When multiple cues appear together, their internal signals largely combine, but the changes in output do not simply add up. We further show that removing the internal signal associated with one cue can suppress its influence, often more effectively than asking the model to ignore demographics via prompting, while largely preserving general benchmark performance. However, the ability to selectively remove one dimension's influence while leaving co-present dimensions intact remains highly model- and attribute-specific. These results connect implicit personalization behavior to an internal signal that can be analyzed and causally controlled.

==> latex/table1_ci_car.tex <==
% Auto-generated by phase1_mechanistic/build_table1_stats.py (T0-5). Do not edit.
% DV: CAR (GPT-4o taxonomy-matched category adoption rate).
% Data: canonical phase-1 runs data/results/<model>/phase1_*_<dim>_movies
%   (last 'NEW' dir if any, else last dir), file delta_w_sed_validation.json,
%   <cond> -> dw_vs_car -> contrastive_norm -> pooled -> scatter (per-sample
%   u = DeltaW mean over top-10 NIE eval layers, v = behavioral value, n = 50).
% Cell: Pearson r with percentile-bootstrap 95% CI (B=2000, seed 42, pair resampling;
%   resamples with zero variance in u or v -- possible for near-constant CAR -- are
%   dropped, so CIs of near-degenerate CAR cells are conditional and can disagree
%   with the t-test stars; stars are authoritative).
% Stars: Benjamini-Hochberg q over the single family of all 84 scorable
%   (model x condition x DV) cells; ^{*} q<.05, ^{**} q<.01, ^{***} q<.001.
% '--': unscorable cell (dw_vs_car null / constant-zero CAR taxonomy content).
\begin{tabular}{llccccc}
\toprule
Dim.\ & Attribute & llama-3-8b & mistral-7b & qwen3-8b & qwen3-14b & phi-4 \\
\midrule
\multirow{3}{*}{race} & Black & $+0.85^{***}\,[+.74,+.92]$ & $+0.73^{***}\,[+.58,+.84]$ & $+0.83^{***}\,[+.69,+.90]$ & $+0.82^{***}\,[+.71,+.89]$ & $+0.73^{***}\,[+.59,+.84]$ \\
 & Asian & $+0.71^{***}\,[+.59,+.81]$ & $+0.46^{**}\,[+.16,+.69]$ & $+0.80^{***}\,[+.59,+.90]$ & $+0.67^{***}\,[+.34,+.82]$ & $+0.35^{*}\,[+.07,+.59]$ \\
 & White & -- & -- & -- & $-0.17\,[-.40,+.08]$ & -- \\
\midrule
\multirow{2}{*}{gender} & Male & $+0.68^{***}\,[+.43,+.83]$ & $-0.27\,[-.74,+.28]$ & $+0.63^{***}\,[+.42,+.77]$ & $+0.45^{**}\,[+.23,+.62]$ & $+0.37^{*}\,[-.21,+.68]$ \\
 & Female & $+0.66^{***}\,[+.17,+.84]$ & $+0.19\,[+.15,+.38]$ & $+0.63^{***}\,[-.07,+.86]$ & $+0.71^{***}\,[+.40,+.85]$ & $+0.30\,[-.05,+.55]$ \\
\midrule
\multirow{4}{*}{age} & Child & $+0.69^{***}\,[+.48,+.80]$ & $+0.50^{***}\,[+.33,+.65]$ & $+0.84^{***}\,[+.77,+.90]$ & $+0.60^{***}\,[+.36,+.75]$ & $+0.51^{***}\,[+.30,+.67]$ \\
 & Adol.\ & $+0.60^{***}\,[+.31,+.78]$ & $+0.05\,[+.00,+.13]$ & -- & $+0.18\,[+.15,+.36]$ & -- \\
 & Adult & $+0.38^{*}\,[+.02,+.64]$ & $-0.06\,[-.12,-.03]$ & $+0.27\,[+.09,+.45]$ & $-0.02\,[-.32,+.30]$ & $+0.02\,[-.24,+.26]$ \\
 & Older & $+0.30\,[-.03,+.53]$ & $+0.55^{***}\,[+.26,+.78]$ & $+0.41^{**}\,[+.33,+.73]$ & $+0.48^{***}\,[+.24,+.66]$ & $+0.26\,[+.07,+.43]$ \\
\bottomrule
\end{tabular}


==> latex/table1_ci_sed.tex <==
% Auto-generated by phase1_mechanistic/build_table1_stats.py (T0-5). Do not edit.
% DV: behavioral SED (description embeddings, phase-0 paired).
% Data: canonical phase-1 runs data/results/<model>/phase1_*_<dim>_movies
%   (last 'NEW' dir if any, else last dir), file delta_w_sed_validation.json,
%   <cond> -> dw_vs_sed_description -> contrastive_norm -> pooled -> scatter (per-sample
%   u = DeltaW mean over top-10 NIE eval layers, v = behavioral value, n = 50).
% Cell: Pearson r with percentile-bootstrap 95% CI (B=2000, seed 42, pair resampling;
%   resamples with zero variance in u or v -- possible for near-constant CAR -- are
%   dropped, so CIs of near-degenerate CAR cells are conditional and can disagree
%   with the t-test stars; stars are authoritative).
% Stars: Benjamini-Hochberg q over the single family of all 84 scorable
%   (model x condition x DV) cells; ^{*} q<.05, ^{**} q<.01, ^{***} q<.001.
% '--': unscorable cell (dw_vs_car null / constant-zero CAR taxonomy content).
\begin{tabular}{llccccc}
\toprule
Dim.\ & Attribute & llama-3-8b & mistral-7b & qwen3-8b & qwen3-14b & phi-4 \\
\midrule
\multirow{3}{*}{race} & Black & $+0.81^{***}\,[+.69,+.89]$ & $+0.69^{***}\,[+.52,+.82]$ & $+0.70^{***}\,[+.60,+.80]$ & $+0.49^{***}\,[+.27,+.66]$ & $+0.62^{***}\,[+.45,+.75]$ \\
 & Asian & $+0.88^{***}\,[+.80,+.93]$ & $+0.53^{***}\,[+.27,+.74]$ & $+0.38^{*}\,[+.13,+.57]$ & $+0.26\,[-.06,+.51]$ & $+0.26\,[-.04,+.53]$ \\
 & White & $+0.35^{*}\,[+.04,+.58]$ & $+0.28\,[-.01,+.59]$ & $+0.19\,[-.22,+.48]$ & $-0.01\,[-.25,+.26]$ & $+0.30\,[-.03,+.57]$ \\
\midrule
\multirow{2}{*}{gender} & Male & $+0.65^{***}\,[+.44,+.80]$ & $+0.37^{*}\,[-.16,+.65]$ & $+0.38^{*}\,[+.19,+.61]$ & $+0.36^{*}\,[+.13,+.55]$ & $+0.24\,[-.13,+.51]$ \\
 & Female & $+0.56^{***}\,[+.22,+.75]$ & $+0.12\,[-.25,+.36]$ & $+0.27\,[-.09,+.57]$ & $+0.40^{**}\,[+.10,+.63]$ & $+0.37^{*}\,[+.11,+.63]$ \\
\midrule
\multirow{4}{*}{age} & Child & $+0.72^{***}\,[+.49,+.83]$ & $+0.40^{**}\,[+.22,+.57]$ & $+0.56^{***}\,[+.38,+.70]$ & $+0.52^{***}\,[+.17,+.72]$ & $+0.61^{***}\,[+.39,+.75]$ \\
 & Adol.\ & $+0.21\,[-.27,+.59]$ & $+0.02\,[-.22,+.25]$ & $+0.31\,[+.07,+.50]$ & $+0.05\,[-.24,+.33]$ & $+0.06\,[-.22,+.34]$ \\
 & Adult & $+0.17\,[-.30,+.53]$ & $+0.07\,[-.18,+.33]$ & $+0.14\,[-.12,+.41]$ & $+0.08\,[-.21,+.35]$ & $-0.03\,[-.32,+.31]$ \\
 & Older & $+0.32^{*}\,[+.07,+.55]$ & $+0.64^{***}\,[+.34,+.82]$ & $-0.03\,[-.35,+.31]$ & $+0.13\,[-.13,+.42]$ & $+0.24\,[-.04,+.50]$ \\
\bottomrule
\end{tabular}


==> latex/table1_deltaA_ci_car.tex <==
% Raw-DeltaA correlations; neutral-normalized CAR; generated by
% phase1_mechanistic/build_deltaA_table1.py.
% BH family: 80 jointly scorable SED + CAR cells.
\begin{tabular}{llccccc}
\toprule
Dim.\ & Attribute & llama-3-8b & mistral-7b & qwen3-8b & qwen3-14b & phi-4 \\
\midrule
\multirow{3}{*}{race} & Black & $+0.85^{***}\,[+.74,+.92]$ & $+0.72^{***}\,[+.57,+.84]$ & $+0.82^{***}\,[+.69,+.90]$ & $+0.81^{***}\,[+.70,+.89]$ & $+0.75^{***}\,[+.62,+.86]$ \\
 & Asian & $+0.71^{***}\,[+.60,+.81]$ & $+0.42^{**}\,[+.11,+.67]$ & $+0.74^{***}\,[+.48,+.85]$ & $+0.66^{***}\,[+.33,+.82]$ & $+0.36^{*}\,[+.12,+.58]$ \\
 & White & -- & -- & -- & $+0.18\,[-.06,+.44]$ & -- \\
\midrule
\multirow{2}{*}{gender} & Male & $+0.58^{***}\,[+.30,+.76]$ & $-0.16\,[-.53,+.37]$ & $+0.61^{***}\,[+.50,+.75]$ & $+0.32^{*}\,[+.07,+.53]$ & $+0.40^{**}\,[-.11,+.69]$ \\
 & Female & $+0.66^{***}\,[+.17,+.84]$ & -- & $+0.66^{***}\,[-.09,+.88]$ & $+0.69^{***}\,[+.36,+.84]$ & $+0.26\,[-.13,+.56]$ \\
\midrule
\multirow{4}{*}{age} & Child & $+0.65^{***}\,[+.34,+.79]$ & $+0.49^{***}\,[+.32,+.65]$ & $+0.80^{***}\,[+.73,+.87]$ & $+0.59^{***}\,[+.34,+.74]$ & $+0.48^{**}\,[+.27,+.65]$ \\
 & Adol.\ & $+0.58^{***}\,[+.28,+.77]$ & -- & -- & -- & $-0.04\,[-.29,+.19]$ \\
 & Adult & $+0.29\,[-.00,+.53]$ & -- & $+0.11\,[-.11,+.37]$ & $+0.06\,[-.17,+.31]$ & $-0.02\,[-.27,+.25]$ \\
 & Older & $+0.22\,[-.04,+.45]$ & $+0.54^{***}\,[+.24,+.77]$ & -- & $+0.48^{**}\,[+.23,+.66]$ & $+0.27\,[+.09,+.43]$ \\
\bottomrule
\end{tabular}


==> latex/table1_deltaA_ci_sed.tex <==
% Raw-DeltaA correlations; neutral-normalized CAR; generated by
% phase1_mechanistic/build_deltaA_table1.py.
% BH family: 80 jointly scorable SED + CAR cells.
\begin{tabular}{llccccc}
\toprule
Dim.\ & Attribute & llama-3-8b & mistral-7b & qwen3-8b & qwen3-14b & phi-4 \\
\midrule
\multirow{3}{*}{race} & Black & $+0.82^{***}\,[+.69,+.89]$ & $+0.68^{***}\,[+.51,+.82]$ & $+0.70^{***}\,[+.60,+.80]$ & $+0.49^{***}\,[+.26,+.66]$ & $+0.64^{***}\,[+.47,+.76]$ \\
 & Asian & $+0.87^{***}\,[+.80,+.92]$ & $+0.51^{***}\,[+.24,+.73]$ & $+0.38^{*}\,[+.14,+.57]$ & $+0.26\,[-.04,+.52]$ & $+0.26\,[-.04,+.53]$ \\
 & White & $+0.34^{*}\,[+.03,+.58]$ & $+0.29\,[+.01,+.60]$ & $+0.18\,[-.22,+.47]$ & $-0.01\,[-.24,+.27]$ & $+0.30\,[-.03,+.56]$ \\
\midrule
\multirow{2}{*}{gender} & Male & $+0.65^{***}\,[+.44,+.80]$ & $+0.37^{*}\,[-.16,+.66]$ & $+0.37^{*}\,[+.18,+.61]$ & $+0.34^{*}\,[+.11,+.53]$ & $+0.26\,[-.11,+.53]$ \\
 & Female & $+0.56^{***}\,[+.23,+.75]$ & $+0.11\,[-.25,+.35]$ & $+0.27\,[-.11,+.57]$ & $+0.40^{**}\,[+.11,+.63]$ & $+0.37^{*}\,[+.10,+.64]$ \\
\midrule
\multirow{4}{*}{age} & Child & $+0.71^{***}\,[+.49,+.83]$ & $+0.39^{*}\,[+.21,+.56]$ & $+0.56^{***}\,[+.38,+.70]$ & $+0.52^{***}\,[+.17,+.72]$ & $+0.62^{***}\,[+.41,+.75]$ \\
 & Adol.\ & $+0.19\,[-.29,+.58]$ & $+0.02\,[-.22,+.25]$ & $+0.29\,[+.05,+.50]$ & $+0.03\,[-.24,+.29]$ & $+0.07\,[-.21,+.36]$ \\
 & Adult & $+0.17\,[-.28,+.54]$ & $+0.08\,[-.17,+.33]$ & $+0.12\,[-.14,+.40]$ & $+0.04\,[-.24,+.31]$ & $-0.02\,[-.31,+.32]$ \\
 & Older & $+0.32^{*}\,[+.07,+.55]$ & $+0.63^{***}\,[+.33,+.82]$ & $-0.04\,[-.36,+.31]$ & $+0.10\,[-.15,+.39]$ & $+0.26\,[-.01,+.52]$ \\
\bottomrule
\end{tabular}


==> latex/table1_phase1_correlations.tex <==
% Phase 1 per-(model, condition) DeltaW x behavior Pearson r, merged (SED + CAR per model).
% Split value: right-aligned number (r) + fixed-width left star field (l) -> decimal-aligned,
% no star collision, headers center cleanly. Bold = strongest r in that (model, DV) column.
% Stars: * p<.05, ** p<.01, *** p<.001 (two-tailed t on r). -- : no scorable CAR taxonomy.
\setlength{\tabcolsep}{2pt}
\begin{tabular}{ll@{\hspace{6pt}}r@{}l@{\hspace{4pt}}r@{}l@{\hspace{6pt}}r@{}l@{\hspace{4pt}}r@{}l@{\hspace{6pt}}r@{}l@{\hspace{4pt}}r@{}l@{\hspace{6pt}}r@{}l@{\hspace{4pt}}r@{}l@{\hspace{6pt}}r@{}l@{\hspace{4pt}}r@{}l}
\toprule
& \multicolumn{4}{r}{llama-3-8b} & \multicolumn{4}{r}{mistral-7b} & \multicolumn{4}{r}{qwen3-8b} & \multicolumn{4}{r}{qwen3-14b} & \multicolumn{3}{r}{phi-4} \\
\cmidrule(lr){3-6}\cmidrule(lr){7-10}\cmidrule(lr){11-14}\cmidrule(lr){15-18}\cmidrule(lr){19-22}
Dim.\ & Attribute & \multicolumn{2}{c}{SED} & \multicolumn{2}{c}{CAR} & \multicolumn{2}{c}{SED} & \multicolumn{2}{c}{CAR} & \multicolumn{2}{c}{SED} & \multicolumn{2}{c}{CAR} & \multicolumn{2}{c}{SED} & \multicolumn{2}{c}{CAR} & \multicolumn{2}{c}{SED} & \multicolumn{2}{c}{CAR} \\
\midrule
\multirow{3}{*}{race} & Black & +0.81 & \makebox[0.9em][l]{$^{***}$} & \textbf{+0.85} & \makebox[0.9em][l]{$^{***}$} & \textbf{+0.69} & \makebox[0.9em][l]{$^{***}$} & \textbf{+0.73} & \makebox[0.9em][l]{$^{***}$} & \textbf{+0.70} & \makebox[0.9em][l]{$^{***}$} & +0.83 & \makebox[0.9em][l]{$^{***}$} & +0.49 & \makebox[0.9em][l]{$^{***}$} & \textbf{+0.82} & \makebox[0.9em][l]{$^{***}$} & \textbf{+0.62} & \makebox[0.9em][l]{$^{***}$} & \textbf{+0.73} & \makebox[0.9em][l]{$^{***}$} \\
 & Asian & \textbf{+0.88} & \makebox[0.9em][l]{$^{***}$} & +0.75 & \makebox[0.9em][l]{$^{***}$} & +0.53 & \makebox[0.9em][l]{$^{***}$} & +0.46 & \makebox[0.9em][l]{$^{***}$} & +0.38 & \makebox[0.9em][l]{$^{**}$} & +0.80 & \makebox[0.9em][l]{$^{***}$} & +0.26 & \makebox[0.9em][l]{} & +0.67 & \makebox[0.9em][l]{$^{***}$} & +0.26 & \makebox[0.9em][l]{} & +0.35 & \makebox[0.9em][l]{$^{*}$} \\
 & White & +0.35 & \makebox[0.9em][l]{$^{*}$} & +0.24 & \makebox[0.9em][l]{} & +0.28 & \makebox[0.9em][l]{$^{*}$} & -- & \makebox[0.9em][l]{} & +0.19 & \makebox[0.9em][l]{} & -- & \makebox[0.9em][l]{} & -0.01 & \makebox[0.9em][l]{} & -0.17 & \makebox[0.9em][l]{} & +0.30 & \makebox[0.9em][l]{$^{*}$} & -- & \makebox[0.9em][l]{} \\
\midrule
\multirow{2}{*}{gender} & Male & +0.65 & \makebox[0.9em][l]{$^{***}$} & +0.68 & \makebox[0.9em][l]{$^{***}$} & +0.37 & \makebox[0.9em][l]{$^{**}$} & -0.27 & \makebox[0.9em][l]{} & +0.38 & \makebox[0.9em][l]{$^{**}$} & +0.63 & \makebox[0.9em][l]{$^{***}$} & +0.36 & \makebox[0.9em][l]{$^{**}$} & +0.45 & \makebox[0.9em][l]{$^{***}$} & +0.24 & \makebox[0.9em][l]{} & +0.37 & \makebox[0.9em][l]{$^{**}$} \\
 & Female & +0.56 & \makebox[0.9em][l]{$^{***}$} & +0.66 & \makebox[0.9em][l]{$^{***}$} & +0.12 & \makebox[0.9em][l]{} & +0.19 & \makebox[0.9em][l]{} & +0.27 & \makebox[0.9em][l]{$^{*}$} & +0.63 & \makebox[0.9em][l]{$^{***}$} & +0.40 & \makebox[0.9em][l]{$^{**}$} & +0.71 & \makebox[0.9em][l]{$^{***}$} & +0.37 & \makebox[0.9em][l]{$^{**}$} & +0.30 & \makebox[0.9em][l]{$^{*}$} \\
\midrule
\multirow{4}{*}{age} & Child & +0.72 & \makebox[0.9em][l]{$^{***}$} & +0.69 & \makebox[0.9em][l]{$^{***}$} & +0.40 & \makebox[0.9em][l]{$^{**}$} & +0.50 & \makebox[0.9em][l]{$^{***}$} & +0.56 & \makebox[0.9em][l]{$^{***}$} & \textbf{+0.84} & \makebox[0.9em][l]{$^{***}$} & \textbf{+0.52} & \makebox[0.9em][l]{$^{***}$} & +0.60 & \makebox[0.9em][l]{$^{***}$} & +0.61 & \makebox[0.9em][l]{$^{***}$} & +0.51 & \makebox[0.9em][l]{$^{***}$} \\
 & Adol.\ & +0.21 & \makebox[0.9em][l]{} & +0.60 & \makebox[0.9em][l]{$^{***}$} & +0.02 & \makebox[0.9em][l]{} & +0.05 & \makebox[0.9em][l]{} & +0.31 & \makebox[0.9em][l]{$^{*}$} & -- & \makebox[0.9em][l]{} & +0.05 & \makebox[0.9em][l]{} & +0.18 & \makebox[0.9em][l]{} & +0.06 & \makebox[0.9em][l]{} & -- & \makebox[0.9em][l]{} \\
 & Adult & +0.17 & \makebox[0.9em][l]{} & +0.38 & \makebox[0.9em][l]{$^{**}$} & +0.07 & \makebox[0.9em][l]{} & -0.06 & \makebox[0.9em][l]{} & +0.14 & \makebox[0.9em][l]{} & +0.27 & \makebox[0.9em][l]{} & +0.08 & \makebox[0.9em][l]{} & -0.02 & \makebox[0.9em][l]{} & -0.03 & \makebox[0.9em][l]{} & +0.02 & \makebox[0.9em][l]{} \\
 & Older & +0.32 & \makebox[0.9em][l]{$^{*}$} & +0.30 & \makebox[0.9em][l]{$^{*}$} & +0.64 & \makebox[0.9em][l]{$^{***}$} & +0.55 & \makebox[0.9em][l]{$^{***}$} & -0.03 & \makebox[0.9em][l]{} & +0.41 & \makebox[0.9em][l]{$^{**}$} & +0.13 & \makebox[0.9em][l]{} & +0.48 & \makebox[0.9em][l]{$^{***}$} & +0.24 & \makebox[0.9em][l]{} & +0.26 & \makebox[0.9em][l]{} \\
\bottomrule
\end{tabular}


==> latex/table1_phase1_correlations_2.tex <==
% Phase 1 per-(model, condition) DeltaW x behavior Pearson r, merged (SED + CAR per model).
% Split value: right-aligned number (r) + fixed-width left star field (l) -> decimal-aligned,
% no star collision, headers center cleanly. Bold = strongest r in that (model, DV) column.
% Stars: * p<.05, ** p<.01, *** p<.001 (two-tailed t on r). -- : no scorable CAR taxonomy.
\setlength{\tabcolsep}{2pt}
\begin{tabular}{ll@{\hspace{6pt}}r@{}l@{\hspace{4pt}}r@{}l@{\hspace{6pt}}r@{}l@{\hspace{4pt}}r@{}l@{\hspace{6pt}}r@{}l@{\hspace{4pt}}r@{}l@{\hspace{6pt}}r@{}l@{\hspace{4pt}}r@{}l@{\hspace{6pt}}r@{}l@{\hspace{4pt}}r@{}l}
\toprule
& \multicolumn{4}{c}{llama-3-8b} & \multicolumn{4}{c}{mistral-7b} & \multicolumn{4}{c}{qwen3-8b} & \multicolumn{4}{c}{qwen3-14b} & \multicolumn{4}{c}{phi-4} \\
\cmidrule(lr){3-6}\cmidrule(lr){7-10}\cmidrule(lr){11-14}\cmidrule(lr){15-18}\cmidrule(lr){19-22}
Dim.\ & Attribute & \multicolumn{2}{c}{SED} & \multicolumn{2}{c}{CAR} & \multicolumn{2}{c}{SED} & \multicolumn{2}{c}{CAR} & \multicolumn{2}{c}{SED} & \multicolumn{2}{c}{CAR} & \multicolumn{2}{c}{SED} & \multicolumn{2}{c}{CAR} & \multicolumn{2}{c}{SED} & \multicolumn{2}{c}{CAR} \\
\midrule
\multirow{3}{*}{race} & Black & +0.81 & \makebox[0.9em][l]{$^{***}$} & \textbf{+0.85} & \makebox[0.9em][l]{$^{***}$} & \textbf{+0.69} & \makebox[0.9em][l]{$^{***}$} & \textbf{+0.73} & \makebox[0.9em][l]{$^{***}$} & \textbf{+0.70} & \makebox[0.9em][l]{$^{***}$} & +0.83 & \makebox[0.9em][l]{$^{***}$} & +0.49 & \makebox[0.9em][l]{$^{***}$} & \textbf{+0.82} & \makebox[0.9em][l]{$^{***}$} & \textbf{+0.62} & \makebox[0.9em][l]{$^{***}$} & \textbf{+0.73} & \makebox[0.9em][l]{$^{***}$} \\
 & Asian & \textbf{+0.88} & \makebox[0.9em][l]{$^{***}$} & +0.71 & \makebox[0.9em][l]{$^{***}$} & +0.53 & \makebox[0.9em][l]{$^{***}$} & +0.46 & \makebox[0.9em][l]{$^{***}$} & +0.38 & \makebox[0.9em][l]{$^{**}$} & +0.80 & \makebox[0.9em][l]{$^{***}$} & +0.26 & \makebox[0.9em][l]{} & +0.67 & \makebox[0.9em][l]{$^{***}$} & +0.26 & \makebox[0.9em][l]{} & +0.35 & \makebox[0.9em][l]{$^{*}$} \\
 & White & +0.35 & \makebox[0.9em][l]{$^{*}$} & -- & \makebox[0.9em][l]{} & +0.28 & \makebox[0.9em][l]{$^{*}$} & -- & \makebox[0.9em][l]{} & +0.19 & \makebox[0.9em][l]{} & -- & \makebox[0.9em][l]{} & -0.01 & \makebox[0.9em][l]{} & -0.17 & \makebox[0.9em][l]{} & +0.30 & \makebox[0.9em][l]{$^{*}$} & -- & \makebox[0.9em][l]{} \\
\midrule
\multirow{2}{*}{gender} & Male & +0.65 & \makebox[0.9em][l]{$^{***}$} & +0.68 & \makebox[0.9em][l]{$^{***}$} & +0.37 & \makebox[0.9em][l]{$^{**}$} & -0.27 & \makebox[0.9em][l]{} & +0.38 & \makebox[0.9em][l]{$^{**}$} & +0.63 & \makebox[0.9em][l]{$^{***}$} & +0.36 & \makebox[0.9em][l]{$^{**}$} & +0.45 & \makebox[0.9em][l]{$^{***}$} & +0.24 & \makebox[0.9em][l]{} & +0.37 & \makebox[0.9em][l]{$^{**}$} \\
 & Female & +0.56 & \makebox[0.9em][l]{$^{***}$} & +0.66 & \makebox[0.9em][l]{$^{***}$} & +0.12 & \makebox[0.9em][l]{} & +0.19 & \makebox[0.9em][l]{} & +0.27 & \makebox[0.9em][l]{$^{*}$} & +0.63 & \makebox[0.9em][l]{$^{***}$} & +0.40 & \makebox[0.9em][l]{$^{**}$} & +0.71 & \makebox[0.9em][l]{$^{***}$} & +0.37 & \makebox[0.9em][l]{$^{**}$} & +0.30 & \makebox[0.9em][l]{$^{*}$} \\
\midrule
\multirow{4}{*}{age} & Child & +0.72 & \makebox[0.9em][l]{$^{***}$} & +0.69 & \makebox[0.9em][l]{$^{***}$} & +0.40 & \makebox[0.9em][l]{$^{**}$} & +0.50 & \makebox[0.9em][l]{$^{***}$} & +0.56 & \makebox[0.9em][l]{$^{***}$} & \textbf{+0.84} & \makebox[0.9em][l]{$^{***}$} & \textbf{+0.52} & \makebox[0.9em][l]{$^{***}$} & +0.60 & \makebox[0.9em][l]{$^{***}$} & +0.61 & \makebox[0.9em][l]{$^{***}$} & +0.51 & \makebox[0.9em][l]{$^{***}$} \\
 & Adol.\ & +0.21 & \makebox[0.9em][l]{} & +0.60 & \makebox[0.9em][l]{$^{***}$} & +0.02 & \makebox[0.9em][l]{} & +0.05 & \makebox[0.9em][l]{} & +0.31 & \makebox[0.9em][l]{$^{*}$} & -- & \makebox[0.9em][l]{} & +0.05 & \makebox[0.9em][l]{} & +0.18 & \makebox[0.9em][l]{} & +0.06 & \makebox[0.9em][l]{} & -- & \makebox[0.9em][l]{} \\
 & Adult & +0.17 & \makebox[0.9em][l]{} & +0.38 & \makebox[0.9em][l]{$^{**}$} & +0.07 & \makebox[0.9em][l]{} & -0.06 & \makebox[0.9em][l]{} & +0.14 & \makebox[0.9em][l]{} & +0.27 & \makebox[0.9em][l]{} & +0.08 & \makebox[0.9em][l]{} & -0.02 & \makebox[0.9em][l]{} & -0.03 & \makebox[0.9em][l]{} & +0.02 & \makebox[0.9em][l]{} \\
 & Older & +0.32 & \makebox[0.9em][l]{$^{*}$} & +0.30 & \makebox[0.9em][l]{$^{*}$} & +0.64 & \makebox[0.9em][l]{$^{***}$} & +0.55 & \makebox[0.9em][l]{$^{***}$} & -0.03 & \makebox[0.9em][l]{} & +0.41 & \makebox[0.9em][l]{$^{**}$} & +0.13 & \makebox[0.9em][l]{} & +0.48 & \makebox[0.9em][l]{$^{***}$} & +0.24 & \makebox[0.9em][l]{} & +0.26 & \makebox[0.9em][l]{} \\
\bottomrule
\end{tabular}


==> latex/table2_ablation_both_sides.tex <==
% Phase 4 ablation grid — vk=dim, desc-SED, both ablation targets per pair.
% Model and Pair merged with \multirow; ratio (ablation vs prompt baseline) bold.
% Stars on Delta_pure(t): * p<.05, ** p<.01, *** p<.001 (one-sided t on per-sample paired Delta).
% dagger: prompt moved the response toward the cue, so the ratio is undefined.  --: no ablation effect.
\begin{tabular}{ll l c r r r r}
\toprule
Model & Pair & target & $\alpha^\star$ & $\Delta_{\rm pure(t)}$ & $d$ & Prompt~$\Delta$ & Ratio \\
\midrule
\multirow{6}{*}{\textbf{llama-3-8b}}
 & \multirow{2}{*}{race\,$\times$\,gender} & race   & 5.0 & $+0.086^{***}$ & $+0.56$ & $+0.006$ & \textbf{13.5$\times$} \\
 &                                         & gender & 4.0 & $+0.005$       & $+0.05$ & $+0.004$ & \textbf{1.2$\times$} \\
\addlinespace[1pt]
 & \multirow{2}{*}{race\,$\times$\,age}    & race   & 5.0 & $+0.078^{***}$ & $+0.54$ & $+0.016$ & \textbf{5.0$\times$} \\
 &                                         & age    & 5.0 & $+0.022^{***}$ & $+0.19$ & $+0.016$ & \textbf{1.4$\times$} \\
\addlinespace[1pt]
 & \multirow{2}{*}{gender\,$\times$\,age}  & gender & 4.0 & $+0.003$       & $+0.03$ & $+0.017$ & \textbf{0.2$\times$} \\
 &                                         & age    & 5.0 & $+0.038^{***}$ & $+0.33$ & $+0.009$ & \textbf{4.5$\times$} \\
\midrule
\multirow{6}{*}{\textbf{mistral-7b}}
 & \multirow{2}{*}{race\,$\times$\,gender} & race   & 5.0 & $+0.226^{***}$ & $+1.59$ & $-0.008$ & $\dagger$ \\
 &                                         & gender & 5.0 & $+0.235^{***}$ & $+1.85$ & $+0.014$ & \textbf{16.7$\times$} \\
\addlinespace[1pt]
 & \multirow{2}{*}{race\,$\times$\,age}    & race   & 5.0 & $+0.154^{***}$ & $+1.22$ & $-0.005$ & $\dagger$ \\
 &                                         & age    & 5.0 & $+0.169^{***}$ & $+1.13$ & $+0.007$ & \textbf{23.3$\times$} \\
\addlinespace[1pt]
 & \multirow{2}{*}{gender\,$\times$\,age}  & gender & 5.0 & $+0.029^{***}$ & $+0.26$ & $-0.013$ & $\dagger$ \\
 &                                         & age    & 5.0 & $-0.008$       & $-0.08$ & $+0.004$ & -- \\
\midrule
\multirow{6}{*}{\textbf{qwen3-8b}}
 & \multirow{2}{*}{race\,$\times$\,gender} & race   & 5.0 & $+0.176^{***}$ & $+0.72$ & $+0.027$ & \textbf{6.6$\times$} \\
 &                                         & gender & 5.0 & $+0.078^{***}$ & $+0.41$ & $+0.031$ & \textbf{2.5$\times$} \\
\addlinespace[1pt]
 & \multirow{2}{*}{race\,$\times$\,age}    & race   & 5.0 & $+0.306^{***}$ & $+1.04$ & $+0.052$ & \textbf{5.9$\times$} \\
 &                                         & age    & 5.0 & $+0.098^{***}$ & $+0.41$ & $+0.020$ & \textbf{4.8$\times$} \\
\addlinespace[1pt]
 & \multirow{2}{*}{gender\,$\times$\,age}  & gender & 5.0 & $+0.078^{***}$ & $+0.42$ & $+0.028$ & \textbf{2.8$\times$} \\
 &                                         & age    & 5.0 & $+0.055^{***}$ & $+0.24$ & $+0.006$ & \textbf{9.2$\times$} \\
\bottomrule
\end{tabular}


==> latex/table2_ablation_qwen.tex <==
% Main-text ablation table: Qwen3-8B only (showcase model; all six targets
% significant). Values identical to the qwen block of the full grid
% (table2_ablation_both_sides.tex), which the appendix shows for all three
% models. vk=dim, desc-SED. Stars: one-sided t on per-sample paired Delta.
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{l l c r r r r}
\toprule
Pair & target & $\alpha^\star$ & $\Delta_{\rm pure(t)}$ & $d$ & Prompt~$\Delta$ & Ratio \\
\midrule
\multirow{2}{*}{race\,$\times$\,gender} & race   & 5.0 & $+0.176^{***}$ & $+0.72$ & $+0.027$ & \textbf{6.6$\times$} \\
                                        & gender & 5.0 & $+0.078^{***}$ & $+0.41$ & $+0.031$ & \textbf{2.5$\times$} \\
\addlinespace[1pt]
\multirow{2}{*}{race\,$\times$\,age}    & race   & 5.0 & $+0.306^{***}$ & $+1.04$ & $+0.052$ & \textbf{5.9$\times$} \\
                                        & age    & 5.0 & $+0.098^{***}$ & $+0.41$ & $+0.020$ & \textbf{4.8$\times$} \\
\addlinespace[1pt]
\multirow{2}{*}{gender\,$\times$\,age}  & gender & 5.0 & $+0.078^{***}$ & $+0.42$ & $+0.028$ & \textbf{2.8$\times$} \\
                                        & age    & 5.0 & $+0.055^{***}$ & $+0.24$ & $+0.006$ & \textbf{9.2$\times$} \\
\bottomrule
\end{tabular}


==> latex/table_composition_gate_comparison.tex <==
% Raw residual contrast versus same-forward gate projection.
\begin{tabular}{lrrr}
\toprule
Model & raw $\bar\rho$ & gate $\bar\rho$ & gate $-$ raw \\
\midrule
llama-3-8b & 0.699 & 0.709 & +0.009 \\
mistral-7b & 0.671 & 0.675 & +0.004 \\
qwen3-8b & 0.621 & 0.624 & +0.003 \\
qwen3-14b & 0.577 & 0.581 & +0.003 \\
phi-4 & 0.663 & 0.672 & +0.008 \\
\midrule
Overall & 0.646 & 0.652 & +0.006 \\
\bottomrule
\end{tabular}


==> latex/table_decomp_weights.tex <==
% Per-(model, pair) decomposition summary: mean fitted weights
% (alpha, beta) +- SD over all mixed-cell samples at L*, and the
% two-basis fit rho under the own-sample basis, a different
% same-cell sample's basis, and the reliability reference.
% rho columns identical to crosssample_control.json.
% Generated by phase3_multidim/build_appendix_tables.py.
\setlength{\tabcolsep}{4pt}
\begin{tabular}{ll cc ccc}
\toprule
& & \multicolumn{2}{c}{weights} & \multicolumn{3}{c}{fit $\bar\rho$} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-7}
Model & Pair & $\bar\alpha$ & $\bar\beta$ & own & cross & reliab. \\
\midrule
llama-3-8b & race$\times$gender & $0.84\pm0.29$ & $0.81\pm0.24$ & $0.710$ & $0.145$ & $0.103$ \\
 & race$\times$age & $0.88\pm0.24$ & $0.85\pm0.22$ & $0.712$ & $0.153$ & $0.104$ \\
 & gender$\times$age & $0.89\pm0.26$ & $0.91\pm0.28$ & $0.703$ & $0.169$ & $0.127$ \\
\addlinespace[2pt]
mistral-7b & race$\times$gender & $0.85\pm0.19$ & $0.87\pm0.18$ & $0.680$ & $0.167$ & $0.151$ \\
 & race$\times$age & $0.87\pm0.17$ & $0.85\pm0.18$ & $0.677$ & $0.149$ & $0.130$ \\
 & gender$\times$age & $0.87\pm0.17$ & $0.85\pm0.17$ & $0.668$ & $0.116$ & $0.090$ \\
\addlinespace[2pt]
qwen3-8b & race$\times$gender & $0.76\pm0.13$ & $0.79\pm0.11$ & $0.638$ & $0.061$ & $0.049$ \\
 & race$\times$age & $0.77\pm0.11$ & $0.78\pm0.11$ & $0.616$ & $0.054$ & $0.045$ \\
 & gender$\times$age & $0.78\pm0.11$ & $0.78\pm0.11$ & $0.615$ & $0.052$ & $0.043$ \\
\addlinespace[2pt]
qwen3-14b & race$\times$gender & $0.76\pm0.09$ & $0.76\pm0.10$ & $0.578$ & $0.053$ & $0.046$ \\
 & race$\times$age & $0.77\pm0.09$ & $0.77\pm0.08$ & $0.581$ & $0.043$ & $0.037$ \\
 & gender$\times$age & $0.79\pm0.09$ & $0.80\pm0.08$ & $0.579$ & $0.047$ & $0.040$ \\
\addlinespace[2pt]
phi-4 & race$\times$gender & $0.85\pm0.15$ & $0.88\pm0.15$ & $0.680$ & $0.140$ & $0.113$ \\
 & race$\times$age & $0.88\pm0.16$ & $0.85\pm0.16$ & $0.666$ & $0.126$ & $0.099$ \\
 & gender$\times$age & $0.86\pm0.16$ & $0.86\pm0.16$ & $0.669$ & $0.122$ & $0.086$ \\
\bottomrule
\end{tabular}


==> latex/table_decomp_weights_deltaA.tex <==
% Raw residual-contrast decomposition; generated by
% phase3_multidim/build_raw_deltaA_paper_artifacts.py.
\setlength{\tabcolsep}{4pt}
\begin{tabular}{ll cc ccc}
\toprule
& & \multicolumn{2}{c}{weights} & \multicolumn{3}{c}{fit $\bar\rho$} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-7}
Model & Pair & $\bar\alpha$ & $\bar\beta$ & own & wrong sample & other mixed \\
\midrule
llama-3-8b & race$\times$gender & $0.84\pm0.27$ & $0.80\pm0.23$ & $0.699$ & $0.131$ & $0.094$ \\
 & race$\times$age & $0.88\pm0.24$ & $0.85\pm0.21$ & $0.704$ & $0.141$ & $0.096$ \\
 & gender$\times$age & $0.89\pm0.25$ & $0.90\pm0.26$ & $0.695$ & $0.156$ & $0.118$ \\
\addlinespace[2pt]
mistral-7b & race$\times$gender & $0.85\pm0.17$ & $0.86\pm0.16$ & $0.676$ & $0.154$ & $0.142$ \\
 & race$\times$age & $0.87\pm0.16$ & $0.85\pm0.17$ & $0.673$ & $0.134$ & $0.119$ \\
 & gender$\times$age & $0.87\pm0.15$ & $0.85\pm0.16$ & $0.665$ & $0.106$ & $0.083$ \\
\addlinespace[2pt]
qwen3-8b & race$\times$gender & $0.76\pm0.12$ & $0.79\pm0.11$ & $0.636$ & $0.059$ & $0.048$ \\
 & race$\times$age & $0.77\pm0.11$ & $0.78\pm0.11$ & $0.614$ & $0.050$ & $0.042$ \\
 & gender$\times$age & $0.78\pm0.11$ & $0.78\pm0.10$ & $0.615$ & $0.051$ & $0.042$ \\
\addlinespace[2pt]
qwen3-14b & race$\times$gender & $0.76\pm0.09$ & $0.76\pm0.09$ & $0.577$ & $0.048$ & $0.043$ \\
 & race$\times$age & $0.76\pm0.09$ & $0.77\pm0.08$ & $0.578$ & $0.038$ & $0.034$ \\
 & gender$\times$age & $0.78\pm0.09$ & $0.80\pm0.08$ & $0.576$ & $0.042$ & $0.036$ \\
\addlinespace[2pt]
phi-4 & race$\times$gender & $0.85\pm0.14$ & $0.87\pm0.14$ & $0.670$ & $0.117$ & $0.097$ \\
 & race$\times$age & $0.87\pm0.15$ & $0.85\pm0.15$ & $0.658$ & $0.103$ & $0.083$ \\
 & gender$\times$age & $0.86\pm0.14$ & $0.85\pm0.14$ & $0.661$ & $0.097$ & $0.069$ \\
\bottomrule
\end{tabular}


==> latex/table_deltaA_gate_summary.tex <==
% Primary raw activation magnitude versus secondary gate projection.
% Corrected CAR uses cued minus neutral-as-condition.
\begin{tabular}{lccccc}
\toprule
 & \multicolumn{2}{c}{SED} & \multicolumn{2}{c}{CAR} & \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
Model & $r_{\Delta A}$ & $r_{\mathrm{gate}}$ & $r_{\Delta A}$ & $r_{\mathrm{gate}}$ & max $|\Delta r|$ \\
\midrule
Llama-3-8B & 0.517 & 0.518 & 0.567 & 0.570 & 0.025 \\
Mistral-7B & 0.341 & 0.345 & 0.403 & 0.416 & 0.040 \\
Qwen3-8B & 0.315 & 0.323 & 0.624 & 0.625 & 0.027 \\
Qwen3-14B & 0.242 & 0.254 & 0.474 & 0.479 & 0.038 \\
Phi-4 & 0.308 & 0.296 & 0.308 & 0.303 & 0.031 \\
\midrule
Overall & 0.345 & 0.347 & 0.473 & 0.476 & 0.040 \\
\bottomrule
\end{tabular}


==> latex/table_heldout_lstar.tex <==
% T0-4 held-out validation of L* selection (red-team S4).
% Sources: canonical phase-1 runs (data/results/<model>/phase1_*_<dim>_movies,
%   last 'NEW' dir else last): recovery_scores.json (per-sample NIE + D_i,
%   post_attn_jsd), deltaA_spectrum.json (per-sample per-layer normalized
%   raw activation-contrast magnitude),
%   delta_w_sed_validation.json (aligned behavioral SED-description v,
%   published top-10 layers and aligned SED vector).
% r in-sample: Pearson r between mean normalized ||DeltaA|| over the
%   published top-10 NIE layers and v on all n=50 samples (reproduces
%   the corrected raw-DeltaA Table-1 r < 1e-6;
%   the published layer set is also reproduced from NIE with the
%   40th-percentile D_i filter for every condition).
% r held-out: 20 half-splits (seed 0..19) x 2 directions = 40 r values;
%   layers selected on one half (40th-pct D_i filter + mean-NIE top-10
%   within the half), r computed on the disjoint other half; mean +- sd.
% Selection candidate pool = layers 0..31 for all models, matching the
%   published pipeline (identify_layers.py N_LAYERS=32; all published
%   top-10 layers are <= 31 in every model, verified).
% Where recovery lists exclude samples (D_i < 0.005; identity of excluded
%   samples not stored), masked NIE positions are mapped to sample indices
%   by a per-split random order-preserving imputation (selection side only;
%   exact when n_valid = 50). See heldout_lstar_summary.json for n_valid.
% Summary rows (non-Llama): mean over the model's 9 conditions of the
%   in-sample r and of the per-condition held-out means; +- is the SD of
%   the 9 per-condition held-out means.
% Stars on in-sample r: * p<.05, ** p<.01, *** p<.001 (two-tailed, n=50).
\begin{tabular}{llrr}
\toprule
Dim.\ & Attribute & $r$ (in-sample) & $r$ (held-out) \\
\midrule
\multicolumn{4}{l}{llama-3-8b} \\
race & Black & $+0.82^{***}$ & $+0.82 \pm 0.04$ \\
 & Asian & $+0.87^{***}$ & $+0.87 \pm 0.03$ \\
 & White & $+0.34^{*}$ & $+0.33 \pm 0.15$ \\
gender & Male & $+0.65^{***}$ & $+0.65 \pm 0.08$ \\
 & Female & $+0.56^{***}$ & $+0.52 \pm 0.17$ \\
age & Child & $+0.71^{***}$ & $+0.71 \pm 0.09$ \\
 & Adol.\ & $+0.19$ & $+0.15 \pm 0.26$ \\
 & Adult & $+0.17$ & $+0.11 \pm 0.28$ \\
 & Older & $+0.32^{*}$ & $+0.32 \pm 0.13$ \\
\midrule
mistral-7b & mean (9 cond.) & $+0.34$ & $+0.33 \pm 0.24$ \\
qwen3-8b & mean (9 cond.) & $+0.32$ & $+0.31 \pm 0.23$ \\
qwen3-14b & mean (9 cond.) & $+0.24$ & $+0.25 \pm 0.20$ \\
phi-4 & mean (9 cond.) & $+0.31$ & $+0.30 \pm 0.22$ \\
\bottomrule
\end{tabular}


==> latex/table_lstar_ablation.tex <==
\begin{tabular}{llll}
\toprule
Dimension & Llama-3-8B & Mistral-7B & Qwen3-8B \\
\midrule
race & 19, 21, 23, 25, 29--30 & 19, 23, 31 & 29--31 \\
gender & 23, 26, 30 & 19, 31 & 30--31 \\
age & 23--25, 30--31 & 19, 22, 31 & 29--31 \\
\bottomrule
\end{tabular}


==> latex/table_lstar_conditions.tex <==
\begin{tabular}{llllll}
\toprule
Condition & Llama-3-8B & Mistral-7B & Qwen3-8B & Qwen3-14B & Phi-4 \\
\midrule
race: Asian & 19, 21--25, 27--30 & 16, 18--19, 23--25, 28--31 & 17, 23--31 & 4--5, 16, 18--19, 24, 28--31 & 10, 22, 24--31 \\
race: Black & 19--20, 22--28, 30 & 16, 18--19, 21, 23--24, 28--31 & 22--31 & 3--4, 12, 18--19, 24, 26, 28, 30--31 & 8, 21--27, 30--31 \\
race: White & 21--30 & 15--19, 25, 28--31 & 20, 23--31 & 6, 8, 14--15, 18, 26--27, 29--31 & 15, 22--28, 30--31 \\
gender: female & 21--30 & 15--16, 18--19, 21, 25, 28--31 & 20, 23--31 & 1--2, 15, 20, 22, 24, 27, 29--31 & 6, 21--23, 25--28, 30--31 \\
gender: male & 21--30 & 15--19, 25, 28--31 & 22--31 & 12, 14, 16--17, 25--29, 31 & 15, 17, 21--27, 31 \\
age: child & 21--26, 28--31 & 19, 21--25, 27--28, 30--31 & 21, 23--31 & 1, 9, 12, 18, 25--29, 31 & 21--23, 25--31 \\
age: adolescent & 21--30 & 18--19, 21--25, 27, 30--31 & 18, 23--31 & 9, 17, 21, 24--27, 29--31 & 20--27, 30--31 \\
age: adult & 21--30 & 15--19, 25, 28--31 & 19, 23--31 & 6, 8, 14, 17, 21, 23, 25, 27, 30--31 & 12, 20--25, 27, 30--31 \\
age: older adult & 20--28, 30 & 15--16, 18--19, 23, 25, 28--31 & 17, 20, 22, 24--25, 27--31 & 15, 20--23, 25, 27, 29--31 & 20--27, 29--30 \\
\bottomrule
\end{tabular}


==> latex/table_mmlu_capability.tex <==
% MMLU 5-shot, 5 subjects × 100 questions = 500 per (model, condition).
% vk=dim, ablate race direction.
% llama-3-8b row is the --raw_prompt rerun (mmlu_capability_llama_raw.csv,
% 2026-05-31). The original chat-template run scored 0.302 at baseline, i.e.
% chance for 4-option MCQ: the chat template broke few-shot MMLU formatting on
% this model. Mistral and Qwen3 are unaffected and use the original run.
% See PHASE4_PLAN.md:1257.
% Prompt (ignore-race) columns removed from this body table: the +0.100
% movement on qwen3-8b is uniform across all five subjects and consistent
% with a prompt-format artifact, not a capability effect. Full numbers and
% the analysis are in the appendix (sec:app-mmlu).
\begin{tabular}{l|r|rrr}
\toprule
& baseline & \multicolumn{3}{c}{ablation} \\
Model & Acc & $\alpha{=}1$ & $\alpha{=}3$ & $\alpha{=}5$ \\
\midrule
llama-3-8b & 0.704 & 0.702 & 0.698 & 0.698 \\
mistral-7b & 0.616 & 0.614 & 0.616 & 0.616 \\
qwen3-8b   & 0.634 & 0.628 & 0.620 & \textbf{0.606} \\
\bottomrule
\end{tabular}


==> latex/table_offtarget_car.tex <==
% T0-9 off-target CAR under ablation (red-team S15 off-axis).
% Data: data/phase4/<model>/metrics_<pair>_K4_movies_dim[_a<alpha>]_car.json
% (unsuffixed alpha = 1.0), per-sample delta_CAR_A/delta_CAR_B records; vk=dim.
% alpha* per (model, pair, ablated side) recomputed exactly as the published
% Table 4 (build_table4_car: argmin over alphas of mean TARGET delta) and
% validated against paper/tables/table4_car_both_sides.tex (18/18 match to
% <5e-4). dCAR(t): the ablated (target) dimension's mean per-sample delta,
% stars = one-sided Wilcoxon (alternative: ablation lowers it), as published.
% dCAR(p): the PARTNER (off-target) dimension's mean per-sample delta under
% the same ablate arm, stars = TWO-SIDED Wilcoxon. Same per-sample records
% for both columns (paired within record). p<.05/.01/.001 = */**/***.
\begin{tabular}{ll l c r r}
\toprule
Model & Pair & target & $\alpha^\star$ & $\Delta$CAR$_{(t)}$ & $\Delta$CAR$_{(p)}$ \\
\midrule
\multirow{6}{*}{\textbf{llama-3-8b}}
 & \multirow{2}{*}{race\,$\times$\,gender} & race & 2.0 & $-0.030^{*}$ & $+0.002$ \\
 &  & gender & 0.5 & $+0.014$ & $-0.002$ \\
\addlinespace[1pt]
 & \multirow{2}{*}{race\,$\times$\,age} & race & 0.5 & $-0.009$ & $+0.001$ \\
 &  & age & 0.5 & $+0.018$ & $-0.026^{***}$ \\
\addlinespace[1pt]
 & \multirow{2}{*}{gender\,$\times$\,age} & gender & 0.5 & $+0.006$ & $-0.002$ \\
 &  & age & 0.5 & $+0.002$ & $-0.028^{***}$ \\
\midrule
\multirow{6}{*}{\textbf{mistral-7b}}
 & \multirow{2}{*}{race\,$\times$\,gender} & race & 1.0 & $+0.006$ & $-0.009$ \\
 &  & gender & 5.0 & $-0.169^{***}$ & $+0.004$ \\
\addlinespace[1pt]
 & \multirow{2}{*}{race\,$\times$\,age} & race & 0.5 & $+0.001$ & $-0.002$ \\
 &  & age & 0.5 & $-0.002$ & $+0.006$ \\
\addlinespace[1pt]
 & \multirow{2}{*}{gender\,$\times$\,age} & gender & 5.0 & $-0.039^{***}$ & $-0.003$ \\
 &  & age & 5.0 & $-0.024^{***}$ & $+0.027^{***}$ \\
\midrule
\multirow{6}{*}{\textbf{qwen3-8b}}
 & \multirow{2}{*}{race\,$\times$\,gender} & race & 5.0 & $-0.092^{***}$ & $+0.095^{**}$ \\
 &  & gender & 1.0 & $-0.002$ & $+0.026^{***}$ \\
\addlinespace[1pt]
 & \multirow{2}{*}{race\,$\times$\,age} & race & 4.0 & $-0.130^{***}$ & $-0.104^{***}$ \\
 &  & age & 1.0 & $+0.009$ & $+0.005$ \\
\addlinespace[1pt]
 & \multirow{2}{*}{gender\,$\times$\,age} & gender & 5.0 & $-0.030^{**}$ & $-0.128^{***}$ \\
 &  & age & 5.0 & $-0.013$ & $+0.041^{***}$ \\
\bottomrule
\end{tabular}


==> latex/table_oneterm_fit.tex <==
% One-term fit baseline for the 2-basis decomposition (red-team S10b).
% Data: per-sample v_gate vectors in data/phase3/<pair>/K4/<model>/
% vgate_vmlp_movies (mixed / pure_A_matched / pure_B_matched), at the
% canonical-run L* layers (anova.json lstar_used). rho = 1 - ||t - Bc*||
% / ||t|| (least squares), averaged over samples x L* within cell, then
% over cells — identical to the published rho_own pipeline
% (crosssample_control.py); the two-term column reproduces
% crosssample_control.json rho_own to <1e-3.
% Delta = rho_two - max(rho_A-only, rho_B-only).
% Generated by phase3_multidim/build_oneterm_fit.py.
\setlength{\tabcolsep}{5pt}
\begin{tabular}{ll rrrr}
\toprule
Model & Pair & $\bar\rho_{\rm two}$ & $\bar\rho_{A\,\rm only}$ & $\bar\rho_{B\,\rm only}$ & $\Delta$ \\
\midrule
llama-3-8b & race$\times$gender & $+0.710$ & $+0.384$ & $+0.292$ & $+0.326$ \\
 & race$\times$age & $+0.712$ & $+0.383$ & $+0.290$ & $+0.330$ \\
 & gender$\times$age & $+0.703$ & $+0.346$ & $+0.345$ & $+0.357$ \\
\addlinespace[2pt]
mistral-7b & race$\times$gender & $+0.680$ & $+0.399$ & $+0.402$ & $+0.278$ \\
 & race$\times$age & $+0.677$ & $+0.403$ & $+0.380$ & $+0.274$ \\
 & gender$\times$age & $+0.668$ & $+0.368$ & $+0.365$ & $+0.300$ \\
\addlinespace[2pt]
qwen3-8b & race$\times$gender & $+0.638$ & $+0.323$ & $+0.328$ & $+0.310$ \\
 & race$\times$age & $+0.616$ & $+0.322$ & $+0.325$ & $+0.291$ \\
 & gender$\times$age & $+0.615$ & $+0.322$ & $+0.326$ & $+0.288$ \\
\addlinespace[2pt]
qwen3-14b & race$\times$gender & $+0.578$ & $+0.309$ & $+0.310$ & $+0.268$ \\
 & race$\times$age & $+0.581$ & $+0.308$ & $+0.315$ & $+0.266$ \\
 & gender$\times$age & $+0.579$ & $+0.297$ & $+0.309$ & $+0.270$ \\
\addlinespace[2pt]
phi-4 & race$\times$gender & $+0.680$ & $+0.370$ & $+0.372$ & $+0.308$ \\
 & race$\times$age & $+0.666$ & $+0.372$ & $+0.353$ & $+0.294$ \\
 & gender$\times$age & $+0.669$ & $+0.359$ & $+0.362$ & $+0.307$ \\
\bottomrule
\end{tabular}


==> latex/table_orth_modes.tex <==
% ablation mode comparison at α=5, vk=dim, description-SED + CAR.
\begin{tabular}{ll|rrr|rrr|rrr}
\toprule
& & \multicolumn{3}{c|}{$\Delta_{pureA}$ (SED-desc)} & \multicolumn{3}{c|}{$\Delta_{CAR_A}$} & \multicolumn{3}{c}{Sel\_SED} \\
Model & Pair & default & raw & multi & default & raw & multi & default & raw & multi \\
\midrule
llama-3-8b & race $\times$ gender & +0.086 & +0.174 & +0.054 & +0.035 & +0.064 & +0.075 & +0.014 & +0.005 & +0.008 \\
llama-3-8b & race $\times$ age & +0.078 & +0.199 & +0.066 & +0.103 & +0.071 & +0.107 & -0.016 & -0.024 & -0.006 \\
llama-3-8b & gender $\times$ age & +0.002 & +0.030 & +0.008 & +0.030 & +0.085 & -0.006 & -0.006 & -0.004 & +0.007 \\
mistral-7b & race $\times$ gender & +0.226 & +0.105 & +0.208 & +0.290 & +0.028 & +0.361 & -0.008 & -0.021 & -0.011 \\
mistral-7b & race $\times$ age & +0.154 & +0.130 & +0.221 & +0.109 & +0.020 & +0.308 & -0.002 & -0.005 & -0.004 \\
mistral-7b & gender $\times$ age & +0.028 & +0.151 & +0.101 & -0.039 & -0.107 & -0.079 & -0.013 & +0.002 & -0.008 \\
qwen3-8b & race $\times$ gender & +0.176 & +0.473 & +0.199 & -0.092 & -0.127 & -0.109 & -0.017 & -0.027 & -0.020 \\
qwen3-8b & race $\times$ age & +0.306 & +0.523 & +0.212 & -0.127 & -0.142 & -0.124 & +0.014 & +0.017 & +0.018 \\
qwen3-8b & gender $\times$ age & +0.078 & +0.137 & +0.074 & -0.030 & +0.109 & -0.045 & +0.029 & +0.007 & +0.042 \\
\bottomrule
\end{tabular}

==> latex/table_quality_proxies.tex <==
% T0-8 recommendation-quality proxies under steering (red-team S8-utility).
% Data: data/phase4/<model>/responses_<pair>_K4_movies_dim[_a5.0].json,
% pooled over the model's 3 pairs (race_gender, race_age, gender_age); vk=dim.
% Rows: none = un-intervened identity-context arm; ablate = ablate_A+ablate_B
% pooled (alpha as marked); prompt = prompt_A+prompt_B pooled (alpha-independent).
% Columns: Items = mean parsed items per response (parser = CAR pipeline's
% extract_items_from_response, reproduces stored n_items exactly);
% Dist(r) = mean within-response distinct-title ratio; Dist(c) = corpus-level
% distinct/total titles; Overlap = mean fraction of the response's title
% multiset shared with the SAME sample's 'none'-arm response (identity-context
% no-steering baseline; no neutral-context per-sample cache exists offline,
% so this is drift-from-baseline, not drift-from-neutral; '--' for none itself,
% =1 by construction); MedVotes = median TMDB vote_count of recommended titles
% (data/tmdb_cache/movies.json; coverage >=99% of title instances).
% Values are descriptive statistics (unsigned); parse-failure counts were 0
% for every group and model.
\begin{tabular}{ll rrrrr}
\toprule
Model & Intervention & Items & Dist(r) & Dist(c) & Overlap & MedVotes \\
\midrule
\multirow{4}{*}{\textbf{llama-3-8b}} & none & 5.00 & 0.999 & 0.022 & -- & 15981 \\
 & ablate ($\alpha{=}1$) & 5.00 & 0.999 & 0.013 & 0.759 & 15981 \\
 & ablate ($\alpha{=}5$) & 5.00 & 1.000 & 0.016 & 0.529 & 12092 \\
 & prompt & 5.00 & 1.000 & 0.012 & 0.691 & 15981 \\
\midrule
\multirow{4}{*}{\textbf{mistral-7b}} & none & 5.00 & 1.000 & 0.015 & -- & 35541 \\
 & ablate ($\alpha{=}1$) & 5.00 & 1.000 & 0.009 & 0.893 & 35541 \\
 & ablate ($\alpha{=}5$) & 5.00 & 1.000 & 0.013 & 0.586 & 30162 \\
 & prompt & 5.00 & 1.000 & 0.009 & 0.838 & 35541 \\
\midrule
\multirow{4}{*}{\textbf{qwen3-8b}} & none & 5.00 & 1.000 & 0.028 & -- & 16233 \\
 & ablate ($\alpha{=}1$) & 5.00 & 1.000 & 0.024 & 0.780 & 16233 \\
 & ablate ($\alpha{=}5$) & 5.23 & 1.000 & 0.039 & 0.394 & 15981 \\
 & prompt & 5.00 & 1.000 & 0.015 & 0.713 & 16233 \\
\bottomrule
\end{tabular}


==> latex/table_ranking_sensitivity.tex <==
% Table: sensitivity of the NIE layer ranking to patching-analysis choices.
% Source: cached recovery_scores.json (per_sample_recovery_jsd, per_sample_jsd_patched,
%   per_sample_D_i_jsd) and layer_sets.json (canonical L_star) of the canonical
%   phase-1 movies runs per (model, dimension):
%   llama-3-8b/age: phase1_20260424_151855_age_movies
%   llama-3-8b/gender: phase1_20260424_055000_NEW_gender_movies
%   llama-3-8b/race: phase1_20260424_NEW_race_movies
%   mistral-7b/age: phase1_20260426_051249_age_movies
%   mistral-7b/gender: phase1_20260426_050653_gender_movies
%   mistral-7b/race: phase1_20260426_045820_race_movies
%   phi-4/age: phase1_20260430_100123_age_movies
%   phi-4/gender: phase1_20260430_095301_gender_movies
%   phi-4/race: phase1_20260430_094014_race_movies
%   qwen3-14b/age: phase1_20260430_055305_age_movies
%   qwen3-14b/gender: phase1_20260430_054434_gender_movies
%   qwen3-14b/race: phase1_20260430_053107_race_movies
%   qwen3-8b/age: phase1_20260426_083156_age_movies
%   qwen3-8b/gender: phase1_20260426_082527_gender_movies
%   qwen3-8b/race: phase1_20260426_081544_race_movies
% Canonical ranking: top-10 layers by mean clipped NIE over samples with
%   D_i >= 40th percentile (reproduced 45/45 conditions 10/10 vs stored
%   L_star; max |stored - reproduced| layer mean = 0.0e+00).
% Candidate pool: layers 0..31 for all models (identify_layers.py
%   hard-codes N_LAYERS = 32; every stored L_star layer is <= 31, verified).
%   Variants use the same pool so overlap isolates filter/clip sensitivity.
% Variants: P20/P60 = D_i percentile filter at 20/60 (clipped NIE); NC-Pxx =
%   unclipped NIE = 1 - JSD_patched/(D_i + 0.005) (no [0,1] clip), recomputed from
%   stored fields (clip(unclipped) matches stored per-sample NIE to
%   8.3e-05, i.e. JSON rounding), with percentile filter at xx.
% Cells: mean |top-10(variant) intersect top-10(canonical)| over the model's
%   9 conditions (race asian/black/white, gender female/male, age child/
%   adolescent/adult/older_adult), out of 10. Min = worst single
%   (condition, variant) overlap for that model.
% Generated by phase1_mechanistic/build_ranking_sensitivity.py.

\begin{tabular}{lcccccc}
\toprule
Model & P20 & P60 & NC-P40 & NC-P20 & NC-P60 & Min \\
\midrule
Llama-3-8B & 9.9 & 9.9 & 10.0 & 9.9 & 9.9 & 9 \\
Mistral-7B & 9.6 & 9.3 & 9.8 & 9.3 & 9.2 & 8 \\
Qwen3-8B & 9.1 & 9.1 & 9.1 & 8.7 & 8.7 & 7 \\
Qwen3-14B & 7.8 & 7.7 & 9.9 & 7.8 & 7.6 & 6 \\
Phi-4 & 9.2 & 9.2 & 9.7 & 9.2 & 9.1 & 8 \\
\bottomrule
\end{tabular}


==> latex/table_sham_matched.tex <==
% Projection-magnitude-matched sham; generated by
% phase4_steering/build_matched_sham_table.py.
\begin{tabular}{lllcccc}
\toprule
Model & Pair & $\alpha$ & \multicolumn{2}{c}{SED $\Delta_{\mathrm{pure}A}$} & \multicolumn{2}{c}{CAR $\Delta_A$} \\
\cmidrule(lr){4-5} \cmidrule(lr){6-7}
 & & & real & matched sham & real & matched sham \\
\midrule
Qwen3-8B & race $\times$ age & 1 & $+0.080$ [+0.058, +0.101] & $+0.015$ [+0.005, +0.025] & $-0.061$ [-0.070, -0.052] & $+0.009$ [-0.000, +0.018] \\
Qwen3-8B & race $\times$ age & 5 & $+0.304$ [+0.276, +0.332] & $+0.113$ [+0.091, +0.134] & $-0.128$ [-0.140, -0.116] & $+0.014$ [+0.001, +0.027] \\
Qwen3-8B & race $\times$ gender & 1 & $+0.005$ [-0.007, +0.016] & $-0.005$ [-0.013, +0.002] & $-0.018$ [-0.030, -0.007] & $+0.005$ [-0.001, +0.012] \\
Qwen3-8B & race $\times$ gender & 5 & $+0.175$ [+0.144, +0.207] & $+0.027$ [+0.011, +0.043] & $-0.092$ [-0.109, -0.075] & $-0.010$ [-0.024, +0.003] \\
\midrule
Mistral-7B & race $\times$ gender & 1 & $+0.024$ [+0.011, +0.037] & $+0.004$ [-0.004, +0.013] & $+0.005$ [+0.001, +0.010] & $+0.004$ [-0.001, +0.010] \\
Mistral-7B & race $\times$ gender & 5 & $+0.224$ [+0.208, +0.240] & $+0.108$ [+0.092, +0.125] & $+0.291$ [+0.262, +0.319] & $+0.068$ [+0.056, +0.082] \\
\bottomrule
\end{tabular}


==> latex/table_subadditivity.tex <==
% Behavioral sub-additivity on description-SED with the DOSE-MATCHED
% pure basis (pure_A_matched / pure_B_matched), pooled over the three
% pairs per model. p: one-sided t on per-sample residuals
% (observed - predicted < 0).
% Generated by phase3_multidim/build_appendix_tables.py.
\begin{tabular}{l r r r r}
\toprule
Model & slope & \% below & shortfall & $p$ \\
\midrule
llama-3-8b & $0.45$ & $85\%$ & $-38\%$ & $<10^{-155}$ \\
mistral-7b & $0.49$ & $68\%$ & $-28\%$ & $<10^{-37}$ \\
qwen3-8b & $0.39$ & $74\%$ & $-37\%$ & $<10^{-108}$ \\
\bottomrule
\end{tabular}

